Predicting Performance of Software Configurations: There is no Silver Bullet

Many software systems offer configuration options to tailor their functionality and non-functional properties (e.g., performance). Often, users are interested in the (performance-)optimal configuration, but struggle to find it, due to missing information on influences of individual configuration options and their interactions. In the past, various supervised machine-learning techniques have been used to predict the performance of all configurations and to identify the optimal one. In the literature, there is a large number of machine-learning techniques and sampling strategies to select from. It is unclear, though, to what extent they affect prediction accuracy. We have conducted a comparative study regarding the mean prediction accuracy when predicting the performance of all configurations considering 6 machine-learning techniques, 18 sampling strategies, and 6 subject software systems. We found that both the learning technique and the sampling strategy have a strong influence on prediction accuracy. We further observed that some learning techniques (e.g., random forests) outperform other learning techniques (e.g., k-nearest neighbor) in most cases. Moreover, as the prediction accuracy strongly depends on the subject system, there is no combination of a learning technique and sampling strategy that is optimal in all cases, considering the tradeoff between accuracy and measurement overhead, which is in line with the famous no-free-lunch theorem.

==> influenceOfSamplingOnTheLearner.tex <==

\begin{table*}
\caption{Stability of the machine-learning techniques.}
\label{table:compRandom}
\centering
\begin{tabular}{ r r r r r r r r r r r r r r }
\toprule
 &  & \multicolumn{2}{c}{ RFT } & \multicolumn{2}{c}{ kNN } & \multicolumn{2}{c}{ KRR } & \multicolumn{2}{c}{ CART } & \multicolumn{2}{c}{ SMR } & \multicolumn{2}{c}{ SVR } \\
 &   &  RN(50)  &  RN(125)  &  RN(50)  &  RN(125)  &  RN(50)  &  RN(125)  &  RN(50)  &  RN(125)  &  RN(50)  &  RN(125)  &  RN(50)  &  RN(125) \\
\midrule
gemm & RB(OW) & 5.3 & 5.6 & 0.4 & 0.4 & 8.9 & 9.5 & 5.8 & 5.8 & 185.9 & 205.8 & 0.4 & 0.4  \\
 & RB(TW(2)) & 8.5 & 8.5 & 2.8 & 2.7 & 1.8 & 1.8 & 8.8 & 8.6 & 181.1 & 340.9 & 0.3 & 0.3  \\
\vspace{0.1cm}
 & RB(TW(3)) & 0.3 & 0.3 & 2.6 & 2.4 & 0.7 & 0.7 & 0.4 & 0.4 & 49.2 & 381.5 & 0.1 & 0.1  \\
Triangular & RB(OW) & 2.1 & 2.1 & 4.0 & 3.0 & 1.4 & 1.3 & 1.9 & 2.0 & 1.8 & 5.1 & 3.4 & 2.4  \\
 & RB(TW(2)) & 0.8 & 1.0 & 1.7 & 1.1 & 0.7 & 0.4 & 1.0 & 1.1 & 4.4 & 2.1 & 2.5 & 1.0  \\
\vspace{0.1cm}
 & RB(TW(3)) & 1.4 & 1.5 & 3.5 & 2.7 & 1.2 & 1.1 & 1.8 & 1.9 & 2.8 & 1.8 & 3.3 & 2.2  \\
Dune & RB(OW) & 0.7 & 0.5 & 1.2 & 0.7 & 2.8 & 1.8 & 0.9 & 0.5 & 716.8 & 38194.6 & 0.3 & 0.2  \\
\vspace{0.1cm}
 & RB(TW(2)) & 0.6 & 0.4 & 1.2 & 0.5 & 2.5 & 1.6 & 1.0 & 0.4 & 10.9 & 2.5 & 0.2 & 0.1  \\
7z & RB(OW) & 9.2 & 9.6 & 34.0 & 14.7 & 12.1 & 10.5 & 9.5 & 11.7 & 95.4 & 64.6 & 18.0 & 15.7  \\
 & RB(TW(2)) & 0.3 & 0.3 & 33.4 & 14.9 & 13.3 & 11.8 & 0.3 & 0.3 & 36.7 & 23.6 & 18.5 & 15.8  \\
\vspace{0.1cm}
 & RB(TW(3)) & 0.4 & 0.4 & 31.5 & 11.7 & 12.1 & 10.3 & 0.4 & 0.3 & 41.9 & 33.3 & 17.5 & 14.0  \\
HiPAcc & RB(OW) & 1.9 & -- & 5.9 & -- & 4.3 & -- & 1.7 & -- & 28.8 & -- & 3.2 & --  \\
 & RB(TW(2)) & 1.0 & -- & 2.1 & -- & 0.6 & -- & 1.3 & -- & 1.0 & -- & 1.1 & --  \\
\vspace{0.1cm}
 & RB(TW(3)) & 0.3 & -- & 2.2 & -- & 0.5 & -- & 0.3 & -- & 0.3 & -- & 0.8 & --  \\
javaGC & RB(OW) & 10.7 & 12.5 & 17.8 & 15.7 & 8.7 & 10.9 & 15.7 & 14.8 & 332.6 & 302.4 & 18.4 & 17.4  \\
 & RB(TW(2)) & 1.6 & 1.1 & 10.7 & 7.5 & 6.5 & 4.7 & 2.7 & 1.3 & 55.4 & 31.7 & 11.8 & 7.8  \\
\vspace{0.1cm}
 & RB(TW(3)) & 1.6 & 1.1 & 10.7 & 7.5 & 6.5 & 4.7 & 2.6 & 1.4 & 37.7 & 30.4 & 11.8 & 7.8  \\
VP9 & RB(OW) & 7.5 & 6.9 & 51.5 & 31.5 & 36.9 & 25.3 & 12.2 & 12.2 & 561.0 & 434.5 & 87.1 & 78.0  \\
 & RB(TW(2)) & 0.4 & 0.2 & 42.8 & 25.7 & 31.9 & 19.0 & 0.4 & 0.2 & 66.3 & 73.5 & 67.1 & 52.9  \\
\vspace{0.1cm}
 & RB(TW(3)) & 0.4 & 0.2 & 36.6 & 19.4 & 29.7 & NA.0 & 0.3 & 0.2 & 14.1 & 35.3 & 34.2 & 18.7  \\
HSMGP & RB(OW) & 5.9 & 6.1 & 29.6 & 20.1 & 18.1 & 18.0 & 5.7 & 6.1 & 8.1 & 7.3 & 3.0 & 2.9  \\
 & RB(TW(2)) & 0.4 & 0.4 & 8.6 & 4.5 & 2.3 & 0.7 & 0.7 & 0.5 & 0.2 & 0.0 & 1.6 & 0.4  \\
\midrule
average & RB(OW) & 5.4 & 6.2 & 18.1 & 12.3 & 11.6 & 11.0 & 6.7 & 7.6 & 241.3 & 5602.0 & 16.7 & 16.7  \\
 & RB(TW(2)) & 1.7 & 1.7 & 12.9 & 8.1 & 7.4 & 5.7 & 2.0 & 1.8 & 44.5 & 67.8 & 12.9 & 11.2  \\
\vspace{0.1cm}
 & RB(TW(3)) & 0.7 & 0.7 & 14.5 & 8.7 & 8.5 & 4.2 & 1.0 & 0.8 & 24.3 & 96.5 & 11.3 & 8.6  \\
\bottomrule
\end{tabular}
\end{table*}

